Disentangling Hate in Online Memes

Hateful and offensive content detection has been extensively explored in a single modality such as text. However, such toxic information could also be communicated via multimodal content such as online memes. Therefore, detecting multimodal hateful content has recently garnered much attention in academic and industry research communities. This paper aims to contribute to this emerging research topic by proposing DisMultiHate, which is a novel framework that performed the classification of multimodal hateful content. Specifically, DisMultiHate is designed to disentangle target entities in multimodal memes to improve hateful content classification and explainability. We conduct extensive experiments on two publicly available hateful and offensive memes datasets. Our experiment results show that DisMultiHate is able to outperform state-of-the-art unimodal and multimodal baselines in the hateful meme classification task. Empirical case studies were also conducted to demonstrate DisMultiHate's ability to disentangle target entities in memes and ultimately showcase DisMultiHate's explainability of the multimodal hateful content classification task.

==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Conclusion.tex <==
In this paper, we proposed a novel framework, \textsf{DisMultiHate}, which learns and disentangles the representations of hate speech-related target entities, such as race and gender, in memes to improve the hateful content classification. We evaluated \textsf{DisMultiHate} on two publicly available datasets, and our extensive experiments have shown that \textsf{DisMultiHate} outperformed the state-of-the-art baselines. We have conducted case studies to empirically demonstrated \textsf{DisMultiHate}'s ability to disentangle target information in the memes. We have also performed error analysis and discussed some of the limitations of the \textsf{DisMultiHate} model. We will incorporate a more advanced reasoning module in the model for future works and test the model on more hateful meme datasets. Through applying \textsf{DisMultiHate} to disentangle the target in hateful memes, we also hope to raise awareness of the vulnerable groups targeted in hate speeches in real-world datasets.  

%We hope that the actual hateful meme examples illustrated the extent of the social issue and the urgency to develop solutions to moderate such toxic content. 



==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Experiment.tex <==
In this section, we will first describe the settings of experiments conducted to evaluate our \textsf{DisMultiHate} model. Next, we discuss the experiment results and evaluate how \textsf{DisMultiHate} fare against other state-of-the-art baselines. We also conduct case studies to qualitatively analyze \textsf{DisMultiHate}'s ability to identify the targets of hateful memes. Finally, we perform error analysis and discuss the limitations of the \textsf{DisMultiHate} model.

\subsection{Evaluation Setting}
\textbf{Dataset.} We evaluate \textsf{DisMultiHate} and the baseline models on the two publicly available hateful memes classification datasets presented in Section~\ref{sec:dataset}. The train-validation-test split of the dataset are illustrated in Table~\ref{tab:dataset}.

\textbf{Evaluation Metrics.} We adopt the evaluation metrics proposed in the hateful meme dataset papers~\cite{kiela2020hateful,suryawanshi2020multimodal}. Specifically, for the evaluation on FHM dataset~
\cite{kiela2020hateful}, we use Area Under the Receiver Operating Characteristic curve (AUROC) and accuracy score as the evaluation metrics. \citet{suryawanshi2020multimodal} had only reported the F1, precision, and recall on the hateful class when they proposed the MultiOFF dataset~\cite{suryawanshi2020multimodal}. However, we noted that due to class imbalance in hate speech classification, most existing studies \cite{fortuna2018survey,schmidt2017survey} have preferred to use weight metrics to evaluate the classification task. Thus, we adopt weighted F1, weighted precision, and weighted recall as the evaluation metrics for the MultiOFF dataset.

\textbf{Baselines.} We benchmark \textsf{DisMultiHate} against the state-of-the-art multimodal methods that were evaluated on the FHM and MultiOFF datasets. We have also included a unimodal baseline for comparison. Specifically, we applied the pre-trained BERT~\cite{devlin2018bert} to extract text features from the meme's text and feed the extracted text features to a fully connected layer for classification.  %Specifically, we compare with two groups of baselines: (a) methods that were proposed in the original  hateful memes dataset papers~\cite{kiela2020hateful,suryawanshi2020multimodal}, and (b) existing studies' techniques that were evaluated on the two datasets. 

For FHM dataset, we compare with the four best performing multimodal models reported in the original dataset paper~\cite{kiela2020hateful}, namely: \textbf{ViLBERT}~\cite{lu2019vilbert}, \textbf{ViLBERT-CC} (i.e., ViLBERT pre-trained on Conceptual Captions~\cite{sharma2018conceptual}), \textbf{VisualBERT}~\cite{li2019visualbert}, and \textbf{VisualBERT-COCO} (i.e., VisualBERT pre-trained on COCO~\cite{lin2014microsoft}). There are many interesting solutions proposed by the Facebook hateful memes classification challenge participants~\cite{zhu2020enhance,zhou2020multimodal,lippe2020multimodal,zhang2020hateful,muennighoff2020vilio,zhong2020classification}. For our evaluation, we benchmark against the methods explored by the top-performing participant\footnote{https://ai.facebook.com/blog/hateful-memes-challenge-winners/}. Specifically, we benchmark against the methods proposed in Zhu's exploration~\cite{zhu2020enhance}: \textbf{ERNIE-Vil}~\cite{yu2020ernie}, \textbf{UNITER}~\cite{chen2020uniter},  \textbf{VILLNA}~\cite{gan2020large}, and \textbf{VL-BERT}~\cite{su2019vl}. We have reproduced the model using the code\footnote{https://github.com/HimariO/HatefulMemesChallenge} released in \cite{zhu2020enhance}. We also adopt the same data augmentation method proposed in \cite{zhu2020enhance} to enhance the models. Specifically, all the reproduced models are augmented with entity tags retrieved using Google Vision Web Entity Detection, and \textbf{VL-BERT} is also further enhanced with demographic information extracted using FairFace~\cite{karkkainen2019fairface}.

For MultiOFF dataset, we compare with the multimodal methods reported in the dataset paper~\cite{suryawanshi2020multimodal}, namely: \textbf{StackedLSTM+VGG16}, \textbf{BiLSTM+VGG16}, and \textbf{CNNText+VGG16}. For these multimodal baselines, the researchers first extract the image features using VGG16~\cite{simonyan2014very} pre-trained on the ImageNetdataset, and extract text features using various text encoders (e.g., BiLSTM). Subsequently, the extracted image and text features are concatenated before feeding into a classifier for hateful meme classification. As the MultiOFF dataset is relatively new, few studies have benchmarked on this dataset. Therefore, as additional baselines, we reproduced the methods proposed by \citet{zhu2020enhance} on the MultiOFF dataset. 
 
%We follow the evaluation settings as proposed in ~\cite{kiela2020hateful}, which introduces the Facebook Hateful Memes (FHM) dataset. We use the metrics: accuracy and the Area Under the Receiver Operating Characteristic curve (AUROC). 
%{\color{orange}Optional to omit equation or to shorten description to save space (if needed). Accuracy is widely understood.}
%The accuracy evaluates how likely the model gives the correct prediction.
%\begin{equation}
%    \text{Accuracy} = \frac{1}{S}\sum_{s=0}^{S}I(y_s=\hat{y}_s),
%\end{equation}
%where $S$ is the number of testing samples, $y_s$ is the predicted class, $\hat{y}_s$ is the ground-truth class and $I$ is the indicator function. AUROC represents the area under the ROC curve, which plots the true positive rate (TPR) vs. false positive rate (FPR) at different classification thresholds $T$:
%\begin{equation}
%    \text{AUROC} = \int_{-\infty}^{\infty} \text{TPR} (T) \text{FPR}^{'}(T) dT.
%\end{equation}
%In ~\cite{suryawanshi2020multimodal} which introduced the MultiOFF dataset, the authors utilized F1, precision and recall as the evaluation metrics. Since the authors' focus was on detection of the hateful memes, only results of F1, precision and recall on the hateful class were reported. However we observed that due to class-imbalance, F1 on the hateful class can be high while weighted F1 can be extremely low. To compare the 
%different models more thoroughly, we adopted weighted F1, weighted precision and weighted recall in our experiments. The computation of the three scores can be formulated as(?????? change the formulas):
%\begin{align}
%    \text{Precision} = \frac{\text{TP}}{\text{TP+FP}}, \\
%    \text{Precision} = \frac{\text{TP}}{\text{TP+FN}}, \\
%    \text{F1} = \frac{2 \cdot \text{Recall} \cdot \text{Precision}}{\text{Recall} + \text{Precision}}.
%\end{align}
%{\color{orange}Optional to omit equation or to shorten description to save space (if needed). Widely understood.}


\subsection{Experimental Results}
\begin{table}[t]
  \caption{Experimental results on FHM dataset.}
  \label{tab:fhm-result}
  \begin{tabular}{c|cc}
    \hline
    Model & Acc. & AUROC\\
    \hline
    BERT (unimodal) & 58.3 & 64.7  \\\hline
    ViLBERT & 62.2 & 71.1  \\
    VisualBERT & 62.1 & 70.6 \\
    ViLBERT-CC & 61.4 & 70.1 \\
    VisualBERT-COCO & 65.1 & 74.0\\\hline
    ERNIE-VIL & 69.0 & 78.7 \\
    UNITER & 68.6 & 78.0 \\
    VILLNA & 71.2  & 78.5  \\
    VL-BERT & 71.4 & 78.8  \\\hline
    \textsf{DisMultiHate} (w/o disentangle) & 73.6 & 81.4 \\
    \textsf{DisMultiHate} & \textbf{75.8} & \textbf{82.8} \\\hline
\end{tabular}
\end{table}

\begin{table}[t]
  \caption{Experimental results on MultiOFF dataset.}
  \label{tab:off-result}
  \begin{tabular}{c|ccc}
    \hline
    Model & F1 & Precision & Recall \\
    \hline
    BERT (unimodal) & 56.4 & 56.1 & 57.7  \\\hline
    StackedLSTM+VGG16 & 46.3 & 37.3 & 61.1 \\
    BiLSTM+VGG16 & 48.0 & 48.6 & 58.4 \\
    CNNText+VGG16 & 46.3 & 37.3 & 61.1  \\\hline
    ERNIE-VIL & 53.1 & 54.3 & 63.7  \\
    UNITER & 58.1 & 57.8 & 58.4  \\
    VILLNA & 57.3 & 57.1 & 57.6   \\
    VL-BERT & 58.9 & 59.5 & 58.5   \\\hline
    % results of our model applied on MultiOFF dataset
    \textsf{DisMultiHate} (w/o disentangle) &  60.8 & 61.4 & 62.7 \\
    \textsf{DisMultiHate}  & \textbf{64.6} & \textbf{64.5} & \textbf{65.1}   \\\hline
\end{tabular}
\end{table}
We have also included a variant of the \textsf{DisMultiHate}, which performed the hateful meme classification without disentangling the target information. Interestingly, we observe that even without the target disentanglement module, \textsf{DisMultiHate} had outperformed the baselines, demonstrating the strength of our data pre-processing approach on augmenting the model with entity and demographics information. \textsf{DisMultiHate} without target disentanglement has also outperformed the VL-BERT model, which was also augmented with entity and demographics. A possible reason for the performance could be due to \textsf{DisMultiHate}'s ability to learn better textual and visual representations for hateful meme classification. Specifically, the visual representation was attended with the textual information, thereby enhancing the visual features with some form of contextual information. Nevertheless, we noted that the performance of target disentanglement further improves the classification results, suggesting the importance of target information in the hateful meme classification task.

Table~\ref{tab:fhm-result} and \ref{tab:off-result} show the experimental results on the FHM and MultiOFF datasets respectively. In both tables, the highest figures are highlighted in \textbf{bold}. We observed that \textsf{DisMultiHate} outperformed the state-of-the-art baselines in both datasets. \textsf{DisMultiHate} has significantly outperformed the baselines proposed in the original dataset papers. For instance, \textsf{DisMultiHate} has outperformed VisualBERT-COCO by more than 10\% (Acc) on the FHM dataset and outperformed BiLSTM+VGG16 by more than 16\% (F1) on the MultiOFF dataset. \textsf{DisMultiHate} has also outperformed the best baseline by 4\% (Acc) and 5\% (F1) on the FHM and MultiOFF, respectively. We noted that the multimodal methods had outperformed the BERT unimodal baselines in the FHM dataset. However, for the experiment on MultiOFF dataset, we observe that the BERT unimodal baseline is able to achieve competitive performance and outperformed the multimodal baselines proposed in the dataset paper~\cite{suryawanshi2020multimodal}. A possible explanation could be the caption and text information in the MultiOFF memes already contain hateful content. Thus, the unimodal baseline using textual features is able to achieve good performance.

%We replicate the results of previously applied models \cite{zhu2020enhance,zhang2020hateful,sandulescu2020detecting,zhou2020multimodal,velioglu2020detecting,zhong2020classification} on the FHM dataset, followed by also newly applying them to MultiOFF. We compare our model against these competing models on both datasets. We also conducted two ablation experiments to study the efficiency of our model and the necessity of cleaning images.

%\noindent \textbf{Comparison Methods} 
%Table \ref{tab:mem-result} presents our experimental results on the FHM dataset in four parts: (1) performance of official baseline; (2) performance from models involved in the hateful meme competition; (3) performance of recent State-Of-The-Art (SOTA) models; (4) our proposed model. From the second part, it can be seen that, most competition participants adopt the official baseline model or similar multi-modal models such as Oscar and UNITER. The main difference between the models is in the choice of dataset for pretraining. For example, Zhong\cite{zhong2020classification} try to pretrain VisualBERT on CC dataset\cite{sharma2018conceptual}. The first prize winning researchers {\color{orange}(should state model name)}  utilizes third-party libraries to extract external information from images such as race tag and entities. However, shown in third part, we find the models like ERNIE and UNITER can not use the race tag information due to limitation of model itself. They focus on feeding external information to existing models instead of how to efficiently utilize available information. Instead of using extremely huge pretrained model, we design a kind of model which can concentrate on efficiently make use of existing information and create a new SOTA results shown in the last part.

%({\color{orange}Can discuss the performance of SOTA models we vary the info they have, i.e. the S, E, L, R)}

%{\color{orange}(want to talk about VL-BERT (S,E) in 3rd part? About same as prize winning model, but we still beat it, even without disentangling. VL-BERT (S,E) also performs quite well for MultiOff. We can also discuss how much the performance of models drop as we move from FHM to MultiOff -> more things to write.)}



%To verify the robustness and generalization of our approach, we apply our model to MultiOFF dataset. For the sake of fairness, we adopt weighted F1 as the main metric and repeat the experiments of MultiOFF baseline. Besides, to show the effectiveness, we also train SOTA models on MultiOFF dataset and compare them all in Table 3. The first part of Table 3 indicates the results of official baseline on weighted F1 metric. The second part shows the performance of SOTA method of FHM trained on MultiOFF. The last part is our results and shows that, in doth validation set and test set on weighted F1, our method achieve best scores. 

%{\color{orange}(Our model without disentangling already outperforms competing methods. Adding disentangling further improves performance.)} 





%\begin{table}[h!]
%  \caption{Experimental results on FHM dataset. Because labels of test set have not been published by Facebook, and most researchers only compare their models with official baseline on phase 1 validation set, so we also choose this set as standard of comparison. The whole table can be divided into four parts. The first and second parts record performance of parts of official baseline models and competitors' models. The third part shows the reproduction results of the first prize winning solutions. The last part records results of our model.{\color{orange}Need to explain S, E, L, R or include legend. Want to shorten name of winning model? cos dun want to explain CFU, HW, etc}}
%  \label{tab:mem-result}
%  \begin{tabular}{c|cc}
%    \toprule
%    Model & Acc. & AUROC\\
%    \midrule
    % outstanding and most used official baseline, record scores from published paper
%    ViLBERT & 62.2 & 71.1  \\
%    VisualBERT & 62.1 & 70.6 \\
%    ViLBERT-CC & 61.4 & 70.1 \\
%    VisualBERT-COCO & 65.1 & 74.0\\
    % Facebook work:
       % Paper:The Hateful Memes Challenge: Detecting Hate Speech in Multimodal Memes
       % \cite{sharma2018conceptual}
    % CC dataset:
       % paper:Conceptual captions: A cleaned, hypernymed, image alt-text dataset for automatic image captioning
       % \cite{sharma2018conceptual}
    % COCO dataset:
       % paper:Microsoft coco: Common objects in context
       % \cite{lin2014microsoft}
    % description:
       %Official baseline offered by Facebook. This team from Facebook tried multiple approaches including Unimodal, Multimodal(Unimodal Pretraining) and Multimodal(Multimodal Pretraining). Unimodal means models only utilizing text or image. Multimodal(Unimodal Pretraining) means trained on text and image but pretrained on text or image. Multimodal(Multimodal Pretraining) means trained on text and image and pretrained on text and image. This part only records the results of two best and most used models:Visual BERT and VilBERT pretrained multimodally and unimodally. COCO means Ms COCO dataset, CC means Conceptual caption dataset. VilBERT CC means VilBERT pretrained on CC dataset 
    
%    \midrule
%    % outstanding results from competitors, record results from published papers
%    %VisualBERT-CC-MRM & - & 74.0\\
%    %cite:
       %\cite{zhong2020classification}
       %paper:Classification of Multimodal Hate Speech--The Winning Solution of Hateful Memes Challenge
    % description:
       %Find Visual BERT pretrained on CC dataset achieves better performance
    %OSCAR & -  & 77.2 \\
    %UNITER & -  & 77.8 \\
    %ERNIE-ViL Base & - & 78.2\\ 
    %ERNIE-ViL Large & - & 78.8\\ 
    %cite:
       %\cite{muennighoff2020vilio,zhong2020classification}
       %paper:VILIO: STATE-OF-THE-ART VISIO-LINGUISTIC MODELS APPLIED TO HATEFUL MEMES
    %description:
       %Try such hot large scale pretrained multimodels as OSCAR,UNITER and ERNIE.
    %ViLBERT (C \& S) & 65.3 & 75.2\\
    %VisualBERT (C \& S) &  64.3 & 72.9\\
    %cite:
       %\cite{zhang2020hateful,muennighoff2020vilio,zhong2020classification}
       %paper:Hateful Memes Detection via Complementary Visual and Linguistic Networks
    %description:
       %Change the vision input feature and text input feature forms of Visual BERT and VilBERT. C means contextual representation. The image representation V is formed through the fusion of three components in dot addition manner. V = V_ROIs + V_contextual + V_pos. V_ROIs,V_contextual and V_pos denote regions of interest feature, feature extracted by last convolution layer (2048-Dim) of ResNet-152 and 4-D position information of ROI respectively. S means Sembedding.symbol detected by open source tool Spacy to indicate whether the each input token is a keyword. Symbol is set to 0, 2, 1 to denotes that padding word, S-keyword and other sentence tokens, respectively. The final text representation is denoted as follows: L = L_BERT + L_Spacy.
    %UNITER$_\text{CV15+CFU+HW+TOLO}$ & - & 80.7 \\
    %cite
       %\cite{}
       %paper:A Multimodal Framework for the Detection of Hateful Memes
    %desctiption:
       %They picked 91 related hateful tags from YOLO9000 object tags. They detect these tags and adding them to their model as external information. CV means cross validation, split the HM training set into CV folds. CFU means text confounder upsampling method. HW means loss re-weighting approach on the hateful class.
    %YOLO9000
       %Paper:YOLO9000: better, faster, stronger
%    ITC & - & 74.8\\
    %cite
       %\cite{}
       %paper:Multimodal Learning for Hateful Memes Detection
    %description:
       %Extract three kinds of features: image captions extracted from images, text and object regions. Feed these three features into transformer to do cross-attention and get though classifier(MLP) to get answers. What extracts me is that they use back-translator(English-German-English, English-Russian-English) to enrich OCR sentences.
%    \midrule
    %SOTA of FHM dataset(top_rank,first prize winning solutions),reproduce training
%    ERNIE-Vil (S,E)  & 69.6 & 79.0  \\
%    ERNIE-Vil (L,E)  & 69.0 & 78.7 \\
%    UNITER (S,E)  & 71.8 & 77.2 \\
%    UNITER (L,E)  & 68.6 & 78.0 \\
%    Villna (S,E)  & 69.6 & 78.5 \\
%    Villna (L,E)  & 71.2  & 78.5  \\
%    VL-BERT  (S,E) & 70.2 & 80.5 \\
%    VL-BERT (L,E)   & 69.2 & 79.2 \\
%    VL-BERT (L,E,R)  & 71.4 & 78.8 \\
    %cite
       %\cite{zhu2020enhance}
       %paper:Enhance Multimodal Transformer With External Label And In-Domain Pretrain: Hateful Meme Challenge Winning Solution
    %description
       %These method is the first prize winning solution. S,L denotes small size and large size, which means relatively low and high dimension hidden states and relatively more and less  attention heads and hidden layers. E means model utilizes entities. R means model utilizes race and gender tags. Only visualBERT can utilize race tag. All models can utilize entities. Villna means Large-scale adversarial training for vision-and-language representation learning applied on visual bert.
%    \midrule
%    Ours (w/o Disentangling) & 73.6 & 81.4 \\
%    Ours (full) & 75.8 & 82.8 \\
%  \bottomrule
%\end{tabular}
%\end{table}




%\begin{table*}[h!]
%  \caption{Comparison with the baseline models, SOTA of FHM and our models on the \textit{validation} and \textit{test} split of the MultiOFF dataset. We choose weighted F1 as main metric for fair.This table is made up of three parts. We repeat the MultiOFF official baseline experiments using new metric and results are recorded in the first part. The second part shows the results of SOTA of FHM trained on MultiOFF dataset. In the last part, we demonstrate performance of our model.}
%  \label{tab:off-result}
%  \begin{tabular}{c|ccc|ccc}
%    \toprule
%     & \multicolumn{3}{c}{Validation} & \multicolumn{3}{c}{Test} \\\hline\hline
%    Model & F1 & Precision & Recall  & F1 & Precision & Recall \\
%    \midrule
    % Repeat training official baseline model of MultiOFF dataset using new metric weighted F1,weighted precision, weighted recall.Text means that the model only utilizes text. The same as image and multi. Repeat training, not recording.
%    LR (text) & 64.8& 65.8& 65.8& 58.8& 61.1& 58.8  \\
    % description:
       %linear regression
%    NB (text) &61.0 &61.7 &60.8 & 60.6& 61.7&60.4 \\
    % description:
       %Naive Bayes
%    DNN (text) & 54.8& 55.7& 54.3& 54.3 & 56.4 & 54.3  \\
    % description:
       %deep neural network four layers based only on text
%    Stacked LSTM (text) &37.2 &55.3 &43.6 & 38.8&69.8 & 47.0 \\
    % description: 
       %two LSTMs are stacked together. A stacked LSTM has the capability of building a higher representation of the data. As the output of an LSTM layer has been fed as input into the other. In the architecture for this baseline, stacked LSTMs are used as feature extractors before the data is being sent to the classiﬁcation layer. Word embeddings are created using a pre-trained GloVe dataset.
%    BiLSTM (text) & 48.1& 47.0& 51.0& 59.0&58.8 &60.4  \\
    % description: 
       %BidirectionalLSTM(BiLSTM)uses GloVe for word embeddings. Unlike LSTM,BiLSTM saves the past as well as future data sequence stop reserve the context of the targeted word.
%    CNN (text) & 36.0& 48.3& 40.9& 40.2& 61.2&46.3  \\
    % description:
       %CNN approaches are suitable for text as it can be represented in a learnable vector form. As text can be represented in such form, CNN can be relied upon to classify the text data as well
%    VGG16 (image) & 46.3& 37.3& 61.1& 21.8& 15.2& 38.9 \\
    % description:
       %A CNN architecture developed by the Visual Geometry Group (VGG) at the University of Oxford
%    Stacked LSTM + VGG16 (multi) & 46.3& 37.3& 61.1& 46.3& 37.3& 61.1 \\
    % description:
       %VGG16 pre-trained on the ImageNetdataset to extract image features. The same Stacked LSTM approach used to extract text feature. Using Early Fusion Approach, that is, cat text feature and image feature before feeding into classifier.
%    BiLSTM + VGG16 (multi) & 48.4& 50.1& 59.1& 48.0& 48.6& 58.4 \\
    % description:
       %VGG:image feature,BiLSTM:text feature. Early fusion approach(detailed in Stacked LSTM+VGG16)
%    CNNText + VGG16 (multi) & 46.3& 37.3& 61.1& 46.3&37.3&61.1  \\
    % description:
       %VGG:image feature,CNN:text feature. Early fusion approach.
    % cite:
       %\cite{suryawanshi2020multimodal}
       %paper:MultimodalMemeDataset(MultiOFF)forIdentifyingOffensiveContentin ImageandText
    % VGG:
       %paper:Very deep convolutional networks for large-scale image recognition
    % LSTM:
       %paper:Long short-term memory
%    \midrule
    % apply SOTA of FHM to MultiOFF dataset using new metric
%    ERNIE-Vil (S,E)  & 64.0 & 63.8 & 64.2 & 59.1 & 59.1 & 59.2  \\
%    ERNIE-Vil (L,E) & 60.0 & 60.4 & 59.8 & 53.1 & 54.3 & 63.7  \\
%    UNITER (S,E)& 61.8 & 62.4 & 61.6 & 50.8 & 52.4 & 50.0  \\
%    UNITER (L,E) & 64.0 & 63.8 & 64.5 & 58.1 & 57.8 & 58.4  \\
%    Villna (S,E)& 63.3 & 63.8 & 63.1 & 46.3 & 47.6 & 45.5  \\
%    Villna (L,E) & 65.6 & 65.5 & 65.8 & 57.3 & 57.1 & 57.6   \\
%    VL-BERT (S,E)& 60.6 & 60.4 & 61.1 & 63.8 & 63.6 & 63.9   \\
%    VL-BERT (L,E) & 62.2 & 63.2 & 61.7 & 62.0 & 62.2 & 61.9   \\
%    VL-BERT (L,E,R) & 62.9 & 64.1 & 62.4 & 58.9 & 59.5 & 58.5   \\
%    \midrule
    % results of our model applied on MultiOFF dataset
%    Ours (w/o Disentangling) & 64.2 & 64.7 & 65.1 & 60.8 & 61.4 & 62.7 \\
%    Ours (full) & 65.3 & 65.6 & 65.1 & 64.6 & 64.5 & 65.1   \\
%  \bottomrule
%\end{tabular}
%\end{table*}
%\noindent \textbf{Ablation Study} We arranged an ablation experiment on our model to show the necessity of cleaning images. Uncleaned p means all information including image features, entities,race tags and gender tags is extracted from uncleaned images. Uncleaned f means only image features are obtained from unclean images. Through the results, Acc and AUROC are rising alone with the process of cleaning images.{\color{red} I think we also need to evaluate how external data helps in multimodal memes detection. But is it our main contirbution? If so, we will add another set of experiments to help analyze. If not, do we need that ablation study?}

\textbf{Ablation Study}. We also conduct an ablation study to examine the usefulness of entity and demographic information augmented in our \textsf{DisMultiHate} method. Table~\ref{tab:fhm-ablation} and \ref{tab:off-ablation} show the results of the ablation study on FHM and MultiOFF datasets, respectively. We observed that \textsf{DisMultiHate} model augmented with both entity and demographic information had yielded the best performance. 

More interestingly, for the FHM dataset, we observed that without augmenting demographic information yields better performance than without augmenting entity information. However, a different observation is made for \textsf{DisMultiHate} performance on the MultiOFF dataset. Specifically, \textsf{DisMultiHate} not augmented with entity information yields better performance than without augmenting demographic information. The ablation study highlights that the model is highly amenable and adapts to different datasets with varying characteristics.



\begin{table}[t]
  \caption{Ablation study on FHM dataset.}
  \label{tab:fhm-ablation}
  \begin{tabular}{c|cc}
    \hline
    Model & Acc. & AUROC\\\hline
    DisMultiHate (w/o Entity) & 60.6 &68.2  \\
    DisMultiHate (w/o Demo) & 72.8 & 80.8  \\
    DisMultiHate (w/o Entity+Demo) & 62.0  & 70.3 \\\hline
    DisMultiHate  & 75.8 & 82.8 \\\hline
\end{tabular}
\end{table}

\begin{table}[t]
  \caption{Ablation study on MultiOFF dataset.}
  \label{tab:off-ablation}
  \begin{tabular}{c|ccc}
    \hline
    Model & F1 & Precision & Recall \\\hline
    DisMultiHate (w/o Entity) & 62.0 & 64.0 & 63.8\\
    DisMultiHate (w/o Demo) & 60.5& 61.0&61.1 \\
    DisMultiHate (w/o Entity+Demo) & 62.0&62.4 &63.1 \\\hline
    DisMultiHate & 64.6 & 64.5 & 65.1   \\\hline
\end{tabular}
\end{table}



%\begin{table}[t]
%  \caption{Ablation study on FHM dataset.}
%  \label{tab:mem-result-ablation}
%  \begin{tabular}{c|cc}
%    \toprule
%    Model & Acc. & AUROC\\
%    \midrule
%    Ours (uncleaned p) & 69.8 & 78.4 \\
%    Ours (uncleaned f) & 73.2 & 80.4\\
%    \midrule
%    Ours (w/o ed) & 62.0  & 70.3 \\
%    Ours (w/o e) & 60.6 &68.2  \\
%    Ours (w/o d) & 72.8 & 80.8  \\
%    \midrule
%    Ours (w/o Disentangling) & 73.6 & 81.4 \\
%    \midrule
%    Ours (full) & 75.8 & 82.8 \\
%  \bottomrule
%\end{tabular}
%\end{table}


% {\color{red}point out that others use industrial tricks: different loss xxx, but we focus on multimodal reasoning itself}
%\begin{table*}[h!]
%  \caption{Comparison with the state-of-art approaches on the \textit{validation} and \textit{test} split of the MultiOFF dataset.}
%  \label{tab:off-result}
%  \begin{tabular}{c|ccc|ccc}
%    \toprule
%     & \multicolumn{3}{c}{Validation} & \multicolumn{3}{c}{Test} \\\hline\hline
%    Model & F1 & Precision & Recall  & F1 & Precision & Recall \\
%    \midrule
%    Ours (uncleaned p) & 62.1& 62.9&63.8 & 62.4& 63.6&63.8\\
%    Ours (uncleaned f) & 63.5 & 65.5 & 63.1& 58.9& 60.9& 58.4\\
%    \midrule
%    Ours (w/o ed) & 62.8& 65.2& 63.1& 64.0&64.4 &65.1 \\
%    Ours (w/o e) &64.7 &64.8 & 65.8& 65.5 & 65.5 & 66.4\\
%    Ours (w/o d) & 64.8 & 65.1 & 65.8 & 60.5& 61.0&61.1 \\
%    \midrule
%    Ours (w/o Disentangling) & 64.2 & 64.7 & 65.1 & 60.8 & 61.4 & 62.7 \\
%    \midrule
%    Ours (full) & 65.3 & 65.6 & 65.1 & 64.6 & 64.5 & 65.1   \\
%  \bottomrule
%\end{tabular}
%\end{table*}





\subsection{Case Study}
The ability to disentangle target information in memes is a core contribution in our \textsf{DisMultiHate} model, and we aim to evaluate this aspect of the model qualitatively. Working towards this evaluation goal, we design an experiment to retrieve relevant memes for a given target query. Specifically, for a given text query (e.g., ``woman''), we first generate its disentangled latent text representation, $\mathbf{l}_\text{q}$, using the process described in Section~\ref{sec:text}. Next, we compute the cosine similarity between $\mathbf{l}_\text{q}$ and the disentangled latent visual representation $\mathbf{v}_p$ of all memes in the FHM dataset. Finally, we retrieved the top $k$ memes with the highest similarity scores with the given target query. Intuitively, if \textsf{DisMultiHate} model is able to disentangle the target information in memes, we should be able to infer the query target from the retrieved memes qualitatively. For example, given the text query ``woman'', we should expect the top $k$ retrieved memes to include woman-related memes.

\begin{table*}[t!]
  \centering
  \caption{Retrieved memes from FHM dataset for a given target. The headers indicate the correctly predicted labels of the retrieved memes.}
  \label{tab:case}
  \begin{tabular}{|c|c|c|c|c| }
    \hline
    \textbf{Target} & \multicolumn{2}{c|}{\textbf{Hateful}} & \multicolumn{2}{c|}{\textbf{Non-Hateful}} \\\hline
    Woman & \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-woman-1.png}}
	\end{minipage}  &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-woman-6.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-woman-4.png}}
	\end{minipage} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-woman-5.png}}
	\end{minipage}\\\hline
%	Muslim Woman & \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-muw-1.png}}
%	\end{minipage}  &
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-muw-2.png}}
%	\end{minipage} &
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-mum-5.png}}
%	\end{minipage} & \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-muw-4.png}}
%	\end{minipage}\\\hline
	Black Man & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-black-1.png}}
	\end{minipage}  &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-black-2.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-black-3.png}}
	\end{minipage} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{case/case-black-5.png}}
	\end{minipage}\\\hline
    \end{tabular}
\end{table*}

\begin{table*}[h]
  \centering
  \caption{Error analysis of wrongly classified memes from FHM dataset.}
  \label{tab:error}
  \begin{tabular}{|c|c|c|c|c| }
    \hline
    \textbf{Meme} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-woman-non.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-mum-non.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-black-hate1.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-mum-hate.png}}
	\end{minipage}\\\hline
    \textbf{Actual Label} & Non-Hateful & Non-Hateful & Hateful & Hateful\\\hline
    \textbf{Predicted Label} & \color{red} Hateful & \color{red} Hateful & \color{red} Non-Hateful & \color{red} Non-Hateful\\\hline
    \textbf{Disentangled Target} & Woman & Catholics & Black Man & Muslim Woman\\\hline
    \end{tabular}
\end{table*}

Table~\ref{tab:case} shows the retrieved memes for a given target. Specifically, we retrieve the two most relevant hateful and non-hateful memes for the given target query. We can intuitively infer that the retrieved memes are relevant to the given query. For example, the retrieved memes for the query ``Muslim Woman'' are observed to contain Muslim women in hajib. Interestingly, for the query ``Black Man'', we observe that the second meme is retrieved even though the image is in black and white, and it is not obvious that there are African Americans in the image. However, \textsf{DisMultiHate} is still able to disentangle the ``Black Man'' target in the meme by using relevant textual information such as ``\textit{dark}'' and ``\textit{pick cotton}'' to infer contextual information on the slavery of African American. A similar observation is observed for the ``Woman'' target query, where the second meme does not contain any image of a woman but an ape. However, the second meme is also relevant to the target query as \textsf{DisMultiHate} disentangle the ``Woman'' target in the meme by using relevant textual information such as ``\textit{Michelle Obama}'' to infer contextual information on insulting the individual's physical appearance(i.e., a woman) with a picture of an ape. In summary, the case studies presented in Table~\ref{tab:case} has demonstrated \textsf{DisMultiHate}'s ability to disentangle the target in memes using a combination of textual and visual information captured in the memes. Similar observations were also made for other potential hate speech target queries (e.g., Hispanic, Asian, transgender, etc.).

%In this section, we provide qualitative analysis of the proposed model. We concentrate on the effectiveness of adding the disentangled matching module in the proposed model. To show how the module helps, for each meme, we find its most similar meme in the latent space. To be more specific, given a querying mem, we generate its disentangled latent representation $\mathbf{l}_\text{q}$. For disentangled latent representations $\mathbf{l}_k$ any other meme in the dataset, we compute the cosine similarity between $\mathbf{l}_\text{q}$ and $\mathbf{l}_i$ and retrieve the meme with the highest similarity:
%\begin{equation}
%    k^* = \mathop{\arg \max}_k \frac{\mathbf{l}_\text{q} \cdot \mathbf{l}_k}{|\mathbf{l}_\text{q}||\mathbf{l}_k|}.
%\end{equation}
%The $k^*$-th meme is the one that is most similar with the querying meme in the latent space. Table~\ref{tab:vis} illustrates the visualization results of pairs of the querying meme and the retrieved meme. Our proposed model gives correct predictions for all shown querying memes, which are annotated as hateful.

%From visualization, we find out that with the disentangled latent module, the model is more capable for pointing out the target of the memes. In the first row of Table~\ref{tab:vis}, all retrieved memes are hateful which share the same target group as the query memes. For instance, in the first example, both hateful memes are hateful towards Muslim. The querying image contains a Muslim, however, there is no explicit hint in the retrieved image that it is related to Muslim. The interesting thing here is that the two memes are the most similar in the latent space, indicating that the model has the capability of pointing out the target of the meme under different situations. The example on the right hand side of the first row gives another evidence. What's more, the querying meme does not contain any explicit clues that it is talking and targeting at whites. Whereas, the model can still figure out the target in the latent space since its most similar meme in the latent space is also the hateful meme towards at whites. The second row of Table~\ref{tab:vis} gives some examples where the retrieved meme is labeled as non-hate. The case on the right corner of Table~\ref{tab:vis} shows that the same image with different contexts talking about the same group will also be close in the latent space. 

%{\color{red} is it sufficient? the retrieved meme is about white then does it mean that the model can point out the targets?}



%\begin{table*}[h]
%  \centering
%  \caption{Querying memes and their most similar memes in the latent space. The column ``label'' corresponds to the label of the retrieved meme.}
%  \label{tab:vis}
%  \begin{tabular}{ |c|c|c|c|c|c| }
%    \hline
% Querying Meme & Retrieved Meme & Label & Querying Meme & Retrieved Meme & Label \\ \hline
%    \begin{minipage}[b]{0.3\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-1-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.3\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-1-retrieve.pdf}}
%	\end{minipage}
%    & Hate &
    
%    \begin{minipage}[b]{0.5\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-3-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.5\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-3-retrieve.pdf}}
%	\end{minipage}
%    & Hate \\ \hline
%    \begin{minipage}[b]{0.38\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\line%width]{images/vis-2-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.3\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-2-retrieve.pdf}}
%	\end{minipage}
%    & N-Hate &
%    \begin{minipage}[b]{0.5\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-4-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.5\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-4-retrieve.pdf}}
%	\end{minipage}
%    & N-Hate 
%    \\ \hline
%  \end{tabular}
%\end{table*}

\subsection{Error Analysis}
Besides analyzing \textsf{DisMultiHate} quantitatively performance over the state-of-the-art baselines, we are also interested in examining the classification errors of \textsf{DisMultiHate}. Table~\ref{tab:error} illustrates four selected examples of \textsf{DisMultiHate}'s wrongly classified memes. For example, \textsf{DisMultiHate} has classified the first meme to be hateful when the actual label of the meme is non-hateful. A possible reason for this error could be the mention of the keyword ``black'' and the disentangled target being ``woman'', which misled the model to make a wrong prediction. 

Our error analysis also reveals some issues with the FHM dataset. For instance, the second meme is annotated as non-hateful in the dataset. However, upon closer examination of the meme, we could infer some form of discrimination towards the Catholics and Priest, and our \textsf{DisMultiHate} has predicted the meme to be hateful. Another issue of the FHM dataset is the potential noise in the dataset. For example, \textsf{DisMultiHate} has wrongly classified the meme as non-hateful when the content is obviously communicating otherwise. We have checked the FHM dataset and found similar memes (i.e., a meme with a running black man) annotated as non-hateful.
%We have checked the FHM dataset and found similar memes (i.e., showing middle finger) annotated as non-hateful.

\textsf{DisMultiHate} has also wrongly predicted the last meme to be non-hateful as none of the textual keyword, or image features provided the context information that it is hateful. Some form of advance reasoning would be required to understand the hateful context presented in this meme. We could explore adding advanced reasoning modules to classify such memes that require deeper reasoning for future work.




%In this section, we do error analysis to understand the further direction for improving our model. We provide three examples in Table~\ref{tab:error} due to the limitation of space. Memes in the left column are all annotated as hateful however, our model predicts as non-hate.



%\begin{table}[h]
%  \centering
%  \caption{Querying memes and their most similar memes in the latent space.}
%  \label{tab:error}
%  \begin{tabular}{|c|c| }
%    \hline
% Querying Meme & Retrieved Meme \\ \hline
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-6-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-6-retrieve.pdf}}
%	\end{minipage}
%    \\ \hline
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-5-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-5-retrieve.pdf}}
%	\end{minipage}
%    \\ \hline
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-7-query.pdf}}
%	\end{minipage}
%    & 
%    \begin{minipage}[b]{0.35\columnwidth}
%		\centering
%		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{images/vis-7-retrieve.pdf}}
%	\end{minipage}
%    \\ \hline
%  \end{tabular}
%\end{table}

%According to the visualization, we find out that 1) some errors come from detecting the targets of the memes incorrectly; 2) detecting the target correctly does not always result in the correct classification. 

%In the first case shown in Table~\ref{tab:error}, it is targeting \crtext{3k}
%\crcomment{1)is it targeting at 3k? or black people? I'm not quite sure about the intuition behind the meme. The below target is the same case; 2) will they argue that the model fails to extract the target of the retrieved meme (on the right) rather than the meme with wrong prediction (left one)}, whereas the most similar meme in the latent space is targeting at \crtext{refugee}. The reason for the wrong detection of targets may be the lack of training instances. For instance, few training examples are targeting at ``3k''. The second wrong prediction case also falsely regards the target of the meme as ``women'' since it align it with a meme targeting at women. In the the second querying meme, it includes a woman in it, however, the woman has other attributes, to be more specific, a muslim woman. The model fails to extract the trivial attributes of the image as a result fails to understand the targe of the mem.
%Since understanding the target of a meme is essential for hateful meme classification, detecting the target incorrectly harms the performance of multimodal hateful meme detection, leading to wrong classification eventually.

%In the third example in Table~\ref{tab:error}, the model extracts the targets of memes successfully since the retrieved meme has the same target as the target of the querying meme. Even understanding what a meme is targeting at, the model still fails at prediction. A plausible reason is that target understanding is the first step of multimodal hateful meme detection and the task requires the capability of complicated reasoning across modalities. For instance, in order to understand the hatefulness towards black people of the third querying meme, the model needs to fully understand the contradiction from the text of the meme, which involves several rounds of reasoning.

%Therefore, detecting targets of a meme aids in the task of multimodal hateful meme detection while enhancing models' ability of complex reasoning is also of vital importance.

%{\color{orange} Wen Haw: Optional sensitivity analysis (For Rui to consider). Given $k$ targets in latent space, if the performance of disentanglement degrades "gently" as we deviate from $k$, then it indicates the model is still quite robust. If the performance is a sharp drop (e.g. from $k$ to $k$-1, $k$+1), then probably no need to show...}




==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Introduction.tex <==
The proliferation of social media has enabled users to share and spread ideas at a prodigious rate. While the information exchanges in social media platforms may improve an individual’s sense of connectedness with real and virtual communities, these platforms are increasingly exploited for the propagation of hateful content that attacks or uses discriminatory languages targeting a person or a group based on their race, religion, gender, etc. \cite{fortuna2018survey,schmidt2017survey}. The spread of online hate speech has sowed discord among individuals or communities online and resulted in violent hate crimes. Therefore, it is a pressing issue to detect and curb online hateful content.

The existing research on automated hateful content detection has predominantly focused on text-based content \cite{fortuna2018survey,schmidt2017survey}, neglecting multimodal content such as memes. \textit{Memes}, which are images with short texts, are a popular communication form in online social media. Although the memes are typically humorous in nature, they are also increasingly used to spread hate. These hateful memes often target certain communities and or individuals based on race, religion, gender, or physical attributes, by portraying them in a derogatory manner~\cite{kiela2020hateful,suryawanshi2020multimodal,gomez2020exploring}. The hateful memes could also be a greater threat to social peace than text-based online hate speeches due to their viral nature; users could re-post or share these hateful memes in multiple conversations and contexts. 

\begin{figure}[t] 
	\centering
	\setlength{\tabcolsep}{0pt} % Default value: 6pt
	\renewcommand{\arraystretch}{0} % Default value: 1
	\begin{tabular}{ccc}
		\includegraphics[scale = 0.3]{images/introduction_img.png} %&  
        %\includegraphics[scale = 0.55]{images/dt-percentage.pdf} 
	\end{tabular}
	\caption{Example of hateful meme.}
	\label{fig:exmaple}
\end{figure}

To combat the spread of hateful memes, social networking platforms such as Facebook had recently released a large hateful meme dataset as part of a challenge to encourage researchers to submit solutions to perform hateful memes classification~\cite{kiela2020hateful}. The research community has answered this challenge by exploring and proposing multimodal classification models \cite{lippe2020multimodal,velioglu2020detecting,muennighoff2020vilio,zhang2020hateful,das2020detecting,zhou2020multimodal}. Several studies had proposed solutions that focused on innovating the fusion techniques to combine text and visual features extracted from memes to perform the classification tasks~\cite{suryawanshi2020multimodal,kiela2020hateful}. Others have explored fine-tuning large-scale pre-trained multimodal methods to perform hateful memes classification~\cite{kiela2020hateful,lippe2020multimodal,velioglu2020detecting,muennighoff2020vilio,zhang2020hateful,das2020detecting,zhou2020multimodal}. Nevertheless, these existing methods have limited explainability and cannot reason the context embedded in the hateful memes.

Hateful meme classification is a challenging task. Consider an example of a hateful meme illustrated in Figure~\ref{fig:exmaple}; when we examine the text and image as independent features, the content seems normal and benign. However, when we interpret the meme as a whole, the underlying message is very offensive and hateful. Another key element that helped us understand hateful meme is the context illustrated in the memes, and often the target entities (e.g., race, religion, etc.) in the hateful message provide important contextual information. For the example in Figure~\ref{fig:exmaple}, the target entity of the hateful content would be both gender and religion (i.e., female Muslim). Existing multimodal hateful meme classification models are unable to capture such target entity contextual information.

This paper aims to address the research gaps by proposing a novel framework, \textsf{DisMultiHate}, which learns and disentangles the representations of hate speech-related target entities, such as race and gender, in memes to improve the hateful content classification. 
Our framework includes a novel self-supervising training task that enables us to extract the target entities using disentangled latent representations. The disentangled representations serve as contextual information to improve hateful meme classification. 

We summarize this paper's contribution\footnote{Code: https://gitlab.com/bottle\_shop/safe/dismultihate} as follows: (i) We propose a novel multimodal hateful meme classification model called \textsf{DisMultiHate}, which disentangles the representations of hate speech-related target entities to improve performance and explainability of hateful meme classification. (ii) We conduct extensive experiments on two publicly available datasets. Our experiment results show that \textsf{DisMultiHate} consistently outperforms state-of-the-art methods in the hateful meme classification. (iii) We conduct case studies and demonstrated \textsf{DisMultiHate}'s ability to identify target entities in hateful memes, thereby providing contextual explanations for the classification results. 

  


==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Model_2.tex <==
%In this section, we elaborate on the proposed \textbf{Disentangled Hate Speech Detection Model} for the multimodal hateful memes detection task. The overview of the proposed model is illustrated in Figure~\ref{fig:arch}.

\begin{figure*}[t] 
	\centering
	\setlength{\tabcolsep}{0pt} % Default value: 6pt
	\renewcommand{\arraystretch}{0} % Default value: 1
	\begin{tabular}{ccc}
		\includegraphics[scale = 0.5]{images/framework.pdf} %&  
        %\includegraphics[scale = 0.55]{images/dt-percentage.pdf} 
	\end{tabular}
	\caption{Architecture of our \textsf{DisMultiHate} model.}
	\label{fig:arch}
\end{figure*}

%overview of how the model works
%{\color{red} is it okay to say embedding? or representation is better? (embedding is mostly used to denote the input to the encoder?) also to be consistent with the module name: representation learning}

Figure~\ref{fig:arch} illustrates the architectural framework of our proposed \textsf{DisMultiHate} model. Broadly, \textsf{DisMultiHate} consists of three main modules: (a) \textit{data pre-processing}, (b) \textit{text representation learning}, and (c) \textit{visual representation learning}. The details of the data pre-processing module are discussed in Section~\ref{sec:preprocessing}. The goal of the text representation learning module is to learn a disentangled latent representation of the combined textual information output from the data pre-processing module. The details of the text representation learning module will be discussed in Section~\ref{sec:text}. 
The visual representation learning module aims to learn a disentangled latent representation based on the meme's image. The details of the visual representation learning module will be discussed in Section~\ref{sec:visual}. 

A core element in the two learning modules is the process of disentangling the target information from the text and visual representations. Specifically, the latent text and visual representations are projected into a disentangled latent space $\mathcal{D}$, where each latent unit of the disentangled representation represents a probability for a certain category of hate (i.e., religion, gender and race, etc.). For a multimodal meme, disentangled targets from the textual modality and the visual modality should be consistent with each other. Therefore, we introduce a self-supervised matching loss, which constrains the disentangled visual representation to be similar to the disentangled text representation. Finally, the learned text and visual representations will be fed into a regression layer to predict the likelihood of the meme being hateful. The classification process will be discussed in Section \ref{sec:classification}.

%Formally, we define the set of image features as $\mathbf{V}=\{\mathbf{v}_i\}_{i=1}^N$, where $\mathbf{v}_i \in \mathbb{R}^d$ is the feature for the $i$-th detected region using \textit{Faster R-CNN}~\cite{ren2016faster} and $N$ is the number of detected region. The text, which is the concatenation of the text extracted from the meme, detected entities, and demographic information from the data pre-processing stage, will be denoted as $\mathbf{O}=\{\mathbf{o}_j\}_{j=1}^M$, where $\mathbf{o}_j \in \mathbb{R}^{|\mathcal{V}|}$ is the one-hot vector representation for the $j$-th word in the concatenated word sequence of the text, $M$ is the length of the text and $\mathcal{V}$ is the vocabulary. 

\subsection{Text Representation Learning}
\label{sec:text}
This module is designed to learn a disentangled latent representation of the textual information extracted from a meme. The input of the module is the concatenation of the text information output of the data pre-processing step. Specifically, we concatenated the text extracted from the meme, detected entities, and demographic information. Formally, we denote the concatenated text information as $\mathbf{O}=\{\mathbf{o}_j\}_{j=1}^M$, where $\mathbf{o}_j \in \mathbb{R}^{|\mathcal{V}|}$ is the one-hot vector representation for the $j$-th word in the text's word sequence, $M$ is the length of the text, and $\mathcal{V}$ is the vocabulary. 


%This module is designed to learn a disentangled representation of the input text in the latent space. First of all, the text is encoded by a \textit{text encoder}, which generates textual representations of each word in the text as well as the sentence level representation. The textual representations will be passed to the \textit{visual representation learning} component while the sentence-level representation will be utilized to learn the textual disentangled representation in the latent space by the \textit{text-target disentanglement} component in this module.


%Roy: Describe the text encoding process. The input will be a concatenation of the output from data pre-processing. Use the same naming convention as per what we use in the data pre-processing. The output will be the text embedding, which will be use as input in the visual representation learning module.

\textbf{Text Encoder}. The concatenated text information $\mathbf{O}$ is first fed into a text encoder to generate latent text representations. Since the input text involves words from various domains such as religion, politics, or military, a powerful text encoder is required to capture the semantics in textual information. Bidirectional Encoder Representations from Transformers (BERT)~\cite{devlin2018bert}, which has demonstrated its superiority in various natural language processing (NLP) tasks, is an ideal text encoder for our task. We initialize the BERT with pre-trained weights and fine-tune it with our task. Using the BERT text encoder, we generate the textual representations as follow:
\begin{equation}
    [\mathbf{s}, \mathbf{C}] = \text{BERT}([\mathbf{w}_\text{[CLS]},\mathbf{O}]),
\end{equation}
where $\mathbf{w}_\text{[CLS]}\in \mathbb{R}^{|\mathcal{V}|}$ denotes the one-hot representations for the ``[CLS]'' token, $[\cdot,\cdot]$ is the concatenation operation and $\mathbf{C}=\{\mathbf{c}_j\}_{j=1}^{M}$ is the set of textual representations, and $\mathbf{c}_j \in \mathbb{R}^u$ is the representation for the $j$-th word in the input text $\mathbf{O}$. Similar to ~\cite{devlin2018bert}, we utilize the representation of the ``[CLS]'' token as the sentence representation $\mathbf{s} \in \mathbb{R}^u$.

\textbf{Text-target disentanglement}. The latent text representation generated using the BERT encoder captures rich information on the meme's semantics. However, for our hateful meme classification task, we are interested in contextual information present in the latent text representation, specifically the targets of the hateful content. For example, in Figure~\ref{fig:arch}, we aim to identify ``gender'' as the target entity of the hateful message. Therefore, we need to design a mechanism to disentangle the target information in the latent text representation $\mathbf{s}$. 

%Based on the semantic representation of the whole sentence $\mathbf{s}$, the \textit{text-target disentanglement} component further generates the disentangled latent representation. 

We first transform the the sentence representation $\mathbf{s}$ into a latent space using a linear projection layer:
\begin{equation}
  \mathbf{s}_\text{p} =\mathbf{W}_\text{s} \mathbf{s} +\mathbf{b}_\text{s} ,
\end{equation}
where $\mathbf{W}_\text{s} \in \mathbb{R}^{|\mathcal{D}|\times u}$ and $\mathbf{b}_\text{s} \in \mathbb{R}^{|\mathcal{D}|}$ are parameters to be learnt. 

The goal of latent space disentanglement is to minimize the overlap of information among latent units in the vector. There are many methods that perform latent space disentanglement using regularization terms to minimize the mutual information between latent units~\cite{chen2018isolating,burgess2018understanding,sanchez2020learning}. For our task, we aim to disentangle the projected text representation such that each unit in the latent vector represents a type of hateful meme targets. Noted that we assume that each meme is likely to concentrate on a certain category of hate (i.e., religion, gender, race, etc.) in most cases. To achieve this objective, we adopt a similar approach to~\cite{ma2020disentangled}, where we maximize the likelihood of the target present in the latent text representation while minimizing for the absent targets. Such a discontinuous $\arg\max$ operation can be fulfilled by applying \textit{Straight-Through Gumbel-Softmax} (STGS) function~\cite{jang2016categorical} over $\mathbf{s}_\text{p}$. Specifically, a continuous vector $\mathbf{z} \in \mathbb{R}^{|\mathcal{D}|}$ is first sampled from the Gumbel-Softmax distribution based on $\mathbf{s}_\text{p}$:


%To encourage disentanglement, many methods add regularization terms to minimize mutual information between units. However, in the case of hateful memes, usually a meme concentrate on a certain target group or individuals. We regard the target which the meme is focusing on as the positive case. Similar to~\cite{ma2020disentangled}, we maximize the likelihood of the positive case (force it to be $1$) while minimizing the rest (force them to be $0$). Such discontinuous $\arg\max$ operation is fulfilled by applying \textit{Straight-Through Gumbel-Softmax} (STGS) function~\cite{jang2016categorical} over $\mathbf{s}_\text{p}$.

%When using STGS, a continuous vector $\mathbf{z}$ is sampled from the Gumbel-Softmax distribution based on $\mathbf{s}_\text{p}$ is generated as:
\begin{align}
\label{eq:gumbel}
    u_k &\sim \text{Uniform} (0,1), \\
    g_k &=-\text{log}(-\text{log}(u_k)),\\
    z_k &=\frac{\text{exp}(\text{log}(s_\text{p}^k)+g_k)/\tau}{\sum_{k=1}^{|\mathcal{|D|}|}\text{exp}(\text{log}(s_\text{p})^k+g_k)/\tau},
\end{align}
where $s_\text{p}^k$ is the $k$-th element in $\mathbf{s}_\text{p}$. In the forward pass, the STGS function then transforms the continuous vector sampled from the Gumbel-Softmax distribution into a one-hot vector~\cite{jang2016categorical}:

%In the forward pass, according to the characteristic of the gumbel-softmax distribution, the STGS function transforms the continuous vector sampled from the Gumbel-Softmax distribution into a one-hot vector:
\begin{equation}
    l_\text{s}^k = \left \{ 
    \begin{array}{l}
    1\quad k=\arg\underset{m}{\min} z_m \\
    0 \quad else
    \end{array}
    \right .
\end{equation}
%In the backward pass, the continuous vector is used for error backpropagation. 
Finally, the exploitation of STGS to generate the disentangled text representation can be simplified as:
\begin{equation}
    \mathbf{l}_\text{s} =\text{Gumbel-Softmax} (\mathbf{s}_\text{p}),
\end{equation}
where $\mathbf{l}_\text{s}=\{s_\text{p}^k\}_{k=1}^{|\mathcal{D}|}$ as generated by Equation~\ref{eq:gumbel}. For example, in Figure~\ref{fig:arch}, the disentangled text representation would be a one-hot latent vector where 1 is assigned to the latent unit that represents `woman' (i.e., target). The disentangled text representation $\mathbf{l}_\text{s}$ will be used in the self-supervised matching with the visual disentangled latent representation in section~\ref{sec:visdis}. 

Via learning a disentangled text representation in the projected latent space, we update the text representation $\mathbf{s}$ through the back-propagation process, thus fine-tuning $\mathbf{s}$ to be more representative of the target information. We then use the updated $\mathbf{s}$ for hateful meme classification, as discussed in Section~\ref{sec:classification}.

\subsection{Visual Representation Learning}
\label{sec:visual}
After learning the text representation, we focus on learning the disentangled latent representation in the visual modality. The input of this module is the image features pre-processed using Faster R-CNN~\cite{ren2016faster}. Formally, we define the set of image features as $\mathbf{V}=\{\mathbf{v}_i\}_{i=1}^N$, where $\mathbf{v}_i \in \mathbb{R}^d$ is the feature for the $i$-th detected region using \textit{Faster R-CNN}~\cite{ren2016faster} and $N$ is the number of detected region.

\textbf{Attention-Based Image Encoder}
To enable better interaction between visual and textual modality, we adopted the multi-head attention proposed in~\cite{attentionashish} to learn an attended latent visual representation of the meme. Specifically, we leverage the textual representations $\textbf{C}$ generated by BERT text encoder as guidance to attend the feature map $\mathbf{V}$ and generate the attended visual representation using the attention-based image encoder. The attended visual representation is computed as follow:

%This module uses the textual representations to extract relevant visual information from the image with attention mechanism. To enable better interaction between visual and textual modality, we apply the idea of multi-head attention proposed in~\cite{grondahl2018all} for generation of the attended image feature. Based on the textual representations $\mathbf{C}$ extracted in Section~\ref{sec:text} and the set of image features $\mathbf{V}$, the process of generation of the text-relevant visual feature is computed as:
%Roy: Describe the attention-based image encoding process using the transformer (remember to cite). The output is a interim visual embedding that will be used as input into the representation disentanglement. We need to also explain the intuition for doing this process.
\begin{align}
    \label{eq:second} \mathbf{F}_t &=\text{softmax} (\frac{\mathbf{W}_{\text{q},t}\mathbf{C}(\mathbf{W}_{\text{k},t}\mathbf{V})^T}{\sqrt{q}})\mathbf{\mathbf{W}_{\text{v},t}V} \\
    \tilde{\mathbf{F}} &= \text{Concate}(\{\mathbf{F}_t\}_{t=1}^{q}) \\
    \label{eq:fourth}\mathbf{G} &= \mathbf{W}_{\text{f},1}(\text{Relu}(\mathbf{W}_{\text{f},2}\tilde{\mathbf{F}})+\mathbf{b}_{\text{f},2})+\mathbf{b}_{\text{f},1}\\
    \label{eq:fifth} \tilde{\mathbf{V}} &= \tilde{\mathbf{F}} + \mathbf{G} \\
    \mathbf{v}_\text{att} &= \sum_{m=1}^{M} \tilde{\mathbf{v}}_m,
\end{align}
where $q$ denotes the number of times the dot-attention is computed in the multi-head attention. Specifically, the $t$-th attended image feature $\mathbf{F}_t \in \mathbb{R}^{\frac{u}{q}\times M}$ is generated as shown in Equation~\ref{eq:second}, where $\mathbf{W}_{\text{c},t} \in \mathbb{R}^{\frac{u}{q}\times u}$, $\mathbf{W}_{\text{k},t} \in \mathbb{R}^{\frac{u}{q}\times d}$ and $\mathbf{W}_{\text{v},t} \in \mathbb{R}^{\frac{u}{q}\times d}$ are parameters involved in the $t-th$ computation. The attended image features in different aspects are concatenated in row and generate $\tilde{\mathbf{F}} \in \mathbb{R}^{u\times M}$. Similar to ~\cite{attentionashish}, a residual connection is applied to the attended image features as illustrated in Equation~\ref{eq:fourth} and~\ref{eq:fifth}. Finally, weighted average pool over the attended image features $\tilde{\mathbf{V}}$ results in the attended latent visual representation $\mathbf{v}_\text{att}$.

\textbf{Visual-Target Disentanglement}
\label{sec:visdis}
Although the attended visual representation is generated with an attention mechanism, there is no explicit guidance or supervision signal that forces the model to focus on the image regions that are more relevant to the contextual information (i.e., target entities of hateful memes). For instance, in Figure~\ref{fig:arch}, the visual representation should ideally focus on the image region with the three women and to be aware that the focused region infers the ``gender'' as the target of the hateful meme. To make the visual representation more ``target-aware'', we design a latent space matching mechanism, which aims to disentangle the target information from the visual representation and constraint the disentangled visual representation to be consistent with the disentangled latent text representation. 

%The attended image feature is generated with attention mechanism. However, there is no explicit guidance or supervision signal that forces the model to locate at the text-relevant regions of the image (i.e. three women in Figure~\ref{fig:arch}). On the other hand, target identification is of vital importance to the task hateful meme detection. Therefore, the attended image feature should incorporate target information. 
%Motivated by what mentioned above, we propose to do latent space matching which disentangles the target information from the visual modality and forces the disentangled visual-target representation to be in consistency with the text-target disentangled latent representation. 

Similar to the text-target disentanglement, we first project the visual representation $\mathbf{v}_\text{att}$ into the latent space with a linear projection layer:
%Based on the attended image feature, similar to the learning of textual disentangled latent representation, it will firstly be transformed into the latent space with a linear projection layer:
\begin{equation}
    \mathbf{v}_\text{p}=\mathbf{W}_\text{a}\mathbf{v}_\text{att} + \mathbf{b}_\text{a},
\end{equation}
where $\mathbf{W}_\text{a} \in \mathbb{R}^{|\mathcal{D}|\times u}$ and $\mathbf{b}_\text{a} \in \mathbb{R}^{|\mathcal{D}|}$ are parameters to be learnt.

To disentangle the target information in the visual representation, we introduce a matching loss that constraints $\mathbf{v}_\text{p}$ to be similar to the disentangled text representation $\mathbf{l}_\text{s}$:
\begin{equation}
\label{eq:matching}
    \mathcal{L}_\text{Match} = \sum_{k=1}^{|\mathcal{D}|} l_\text{s}^k log(v_\text{p}^k)+(1-l_\text{s}^k )log(1-v_\text{p}^k),
\end{equation}
where $v_\text{p}^k$ is the $k$-th unit in the visual latent representation $\mathbf{v}_\text{p}$. The matching loss serves as a supervision signal to disentangle the target information in the latent visual representation. The underlying intuition is that the disentangled text representation $\mathbf{l}_\text{s}$ is trained to disentangle the target in the textual information, and constraining the disentangled visual representation to be similar to the disentangled text representation would enable the target latent unit to be maximized in disentangled visual representation. For example, in Figure~\ref{fig:arch}, the matching loss will take guidance from the disentangled text representation and enforce the disentangled visual representation to maximize the latent unit representing ``gender''. 

Similarly to the text representation learning, the visual representation $\mathbf{\mathbf{v}_\text{att}}$ would be updated through the back-propagation process, fine-tuning $\mathbf{v}_\text{att}$ to be more representative of the target information. The updated $\mathbf{v}_\text{att}$ would be used for the hateful meme classification discussed in Section~\ref{sec:classification}.


%Since in order to minimize the matching loss, only the likelihood of the unit corresponds to the target extracted from the text be maximized while the rest will be minimized. On the other hand, the disentanglement target information learned from the attended image feature should be consistent with the target information learned from the text, which serves as a self-supervised signal and ensures the attended visual representation containing correct target information.
%Roy: I have differentiate two types of projections. The text embedding is projected using the linear later follow by the gumbel-softmax. We call this the disentanglement projection. The visual embedding is simply projected to the common latent space using a linear function. This part we will need to explain why the units in disentangled representation would represent the different target. Then we discuss about the disentangled latent representation learning process where a matching loss is used to ensure the visual embedding remain close to the disentangled target embedding, there by resulting in a disentangled visual embedding.  
%The key is to explain the disentanglement



\subsection{Classification}
\label{sec:classification}
To perform hateful meme classification, we leverage a regression layer to generate a \textit{hateful score}. Specifically, if the hateful score is above a threshold, it will be regarded as hateful, otherwise non-hate. By learning the disentangled textual and visual representation and minimizing the matching loss between them in the latent space, the sentence representation $\mathbf{s}$ and the attended image feature $\mathbf{v}_\text{att}$ are both fine-tuned to be more representative of the target information. Finally, we concatenate $\mathbf{s}$ and $\mathbf{v}_\text{att}$, and feed the concatenated representation to a regression layer for the score prediction:
\begin{equation}
    y=\sigma ( \mathbf{w}_\text{r}^T[\mathbf{s},\mathbf{v}_\text{att}] + b_\text{r}),
\end{equation}
where $\mathbf{w}_\text{r} \in \mathbb{R}^{2u}$ and $b_\text{r} \in \mathbb{R}$ are parameters to be learnt. Following~\cite{kiela2020hateful}, we set the threshold $\lambda$ as $0.5$: if the score $y$ is above the threshold, it will be predicted as a hateful meme, otherwise, non-hate. 

%\subsubsection{Loss Function}
\textbf{Loss Function}. We optimize the following loss when training our model using mini-batch gradient descent:
\begin{equation}
    \mathcal{L}_{\bm{\theta}} =  \mathcal{L}_{\bm{\theta},\text{Predict}} + \mu \mathcal{L}_{\bm{\theta},\text{Match}},
\end{equation}
where $\bm{\theta}$ denotes parameters of the model, $\mathcal{L}_{\bm{\theta},\text{Match}}$ is the matching loss in the disentangled latent space, computed from the sum of matching loss over all training samples (see Equation~\ref{eq:matching}); and $\mathcal{L}_{\bm{\theta},\text{Predict}}$ is the loss from prediction and $\mu$ is the hyper-parameter balancing the relative importance of both loss types. 
The prediction loss is defined as:
\begin{equation}
   \mathcal{L}_{\bm{\theta},\text{Predict}} = \sum_{s=1}^{|\mathcal{T}|} \hat{y}_s log(y_s) + (1-\hat{y}_s)log(1-y_s),  
\end{equation}
where $\mathcal{T}$ is the training set and $\hat{y}_s$ is the ground-truth label and $y_s$ is the predicted score of the $s$-th training sample. 

\subsection{Implementation Details}
\label{sec:details}
We set the dimension size to 2048 for image features extracted from Faster R-CNN~\cite{ren2016faster}. All textual information is tokenized using BERT~\cite{devlin2018bert} default tokenizer. The length of the sequence is set to $64$, and shorter sentences are padded while longer sentences are truncated. Weights in the BERT-based model are used to initialize the text encoder. The hyperparameter $\mu$ for balancing prediction loss and matching loss is set to be $0.05$ on the FHM dataset and $0.03$ on the MultiOFF dataset. All implementations are done in Pytorch, and we adopt AdamW~\cite{loshchilov2018fixing} as the optimization algorithm to train our model. The size of the minibatch is set to $64$.  
%When applying the SOTA method of FHM dataset on the MultiOFF dataset, we change nothing except number of train steps, val steps and warm up steps. 
%The length of question latent learning rate dimension of latent space optimizer

==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Preliminary.tex <==
\subsection{Problem Definition}
We define the problem of hateful memes multimodal classification as follows: Given an image $\mathcal{I}$ and a piece of text $\mathcal{O}$ consisting of a sequence of words, a classification model will predict the label of the multimodal meme (\textit{hateful} or \textit{non-hateful}). This binary classification task can also be regarded as a regression task, where a model predicts a confidence score $y \in \mathbb{R}$ ranging from zero to one, indicating the likelihood of the meme being hateful. Specifically, the meme would be regarded as hateful if the predicted score is above a threshold $\lambda$; otherwise, the meme is predicted to be non-hateful.

\subsection{Datasets}
\label{sec:dataset}
We train and evaluate our proposed model on two popular and publicly-available hateful datasets: \textit{Facebook hateful memes (FHM} and \textit{MultiOff}. Table \ref{tab:dataset} shows the distributions of the datasets.

%\begin{table}[t]
%  \caption{Distributions about Facebook Hateful Memes (FHM) and MultiOFF datasets}
%  \label{tab:dataset}
%  \begin{tabular}{c|c|p{14em}}
%    \hline
%    \textbf{Dataset} & \textbf{\#tweets} & \textbf{Classes (\#tweets)}\\\hline\hline
%    FHM & 10,000 & hateful (3800), non-hateful (6200)\\\hline
%    MultiOFF & 743 & offensive (303), non-offensive (440)\\\hline
%\end{tabular}
%\end{table}

\begin{table}[t]
  \caption{Distributions of FHM and MultiOFF datasets}
  \label{tab:dataset}
  \begin{tabular}{c|p{6em}|p{6em}|p{6em}}
    \hline
    \textbf{Dataset}& \textbf{train} &\textbf{validation} & \textbf{test}\\\hline\hline\hline
    FHM & hateful (3050), non-hateful (5450) & hateful (250), non-hateful (250) & hateful (500), non-hateful (500)  \\\hline\hline
    MultiOFF & offensive (187), non-offensive (258) &  offensive (58), non-offensive (91) & offensive (58), non-offensive (91)\\\hline\hline
\end{tabular}
\end{table}




\textbf{Facebook Hateful Memes (FHM)}~\cite{kiela2020hateful}:
The dataset was constructed and released by Facebook as part of a challenge to crowd-source multimodal hateful meme classification solutions. The dataset contains $10K$ memes with binary labels(i.e., hateful or non-hateful). The Facebook challenge did not release the labels of the memes in the test split. Therefore, we utilize the \textit{dev-seen} split as the \textit{test}. Existing studies have also adopted the same dataset setting in their training and evaluations~\cite{lippe2020multimodal,zhou2020multimodal,zhu2020enhance}.

\textbf{MultiOFF}~\cite{suryawanshi2020multimodal}: The dataset contains $1K$ memes related to the 2016 United States presidential election. The memes are labeled as \textit{offensive} or \textit{non-offensive}. Although the authors have labeled the memes based on offensiveness, we manually examined the memes and found that the offensive memes could also be considered hateful as most of them contain abusive and discriminatory messages against a person or minority group. 


%It collects and annotated around $1$k memes related to the 2016 U.S. presidential election and creates a multimodal meme dataset. The memes are categorised as \textit{offensive} and \textit{non-offensive}. Correct classification of memes asks for the alignment between visual and textual modalities and the comprehension of both modalities.
%Memes will be deemed offensive if they intend the following: personal attack, homophobic abuse, racial abuse, or attack on minority. Following this definition together with the definition in~\cite{waseem2016hateful,ParkF17,DavidsonWMW17}, we reformulate \textit{offensive} memes as \textit{hateful} memes while \textit{non-offensive} ones as \textit{non-hate} memes.
%We use the provided \textit{val} split for validation and evaluate models with the \textit{test} split when they achieves the best performance on the \textit{val} split.


%This dataset is focusing on hate speech detection in the multimodal setting. It is constructed manually such that truly multimodal reasoning and understanding is required and only multimodal models can succeed.  The dataset contains $10$k memes in total and formulates multimodal hateul memes detection into a binary classification task, on which most the state-of-the-art methods perform poorly (around $60\%$ accuracy). Since the labels of the test split in the dataset are not availabel, we use \textit{dev-seen} split as the \textit{test} set following most of previous works. The \textit{dev-seen} split is fully balanced, $80\%$ of its hateful memes are \textit{multimodal hate}, where benign confounders can be found for both modalities, while the rest hateful memes are \textit{unimodal hate}. Among non-hate memes in \textit{dev-seen}, $80\%$ contains either \textit{benign image} or \textit{benign text} confounders, and the rest are random non-hateful.

%{\color{red} the author defined the mems as offensive and non-offensive in the original paper. but we utilize them as hate vs. non-hate. Is the explanation provided in the following part reasoning for such usage?}

%\noindent \textbf{MultiOFF}~\cite{suryawanshi2020multimodal}: It collects and annotated around $1$k memes related to the 2016 U.S. presidential election and creates a multimodal meme dataset. The memes are categorised as \textit{offensive} and \textit{non-offensive}. Correct classification of memes asks for the alignment between visual and textual modalities and the comprehension of both modalities.
%Memes will be deemed offensive if they intend the following: personal attack, homophobic abuse, racial abuse, or attack on minority. Following this definition together with the definition in~\cite{waseem2016hateful,ParkF17,DavidsonWMW17}, we reformulate \textit{offensive} memes as \textit{hateful} memes while \textit{non-offensive} ones as \textit{non-hate} memes.
%We use the provided \textit{val} split for validation and evaluate models with the \textit{test} split when they achieves the best performance on the \textit{val} split.


\subsection{Data Pre-processing}
\label{sec:preprocessing}
To improve our proposed method's reproducibility, we also provide an overview of the data pre-processing steps applied on the FHM and MultiOFF memes datasets. Specifically, the following steps were taken to pre-process the memes in the datasets:

\begin{itemize}
    \item \textbf{Image resizing}: The datasets provided memes in all sizes. We resized the images proportionally to a minimum of 140 pixels and a maximum of 850 pixels. This ensures consistency of the visual input into our proposed model and baselines.
    \item \textbf{Text extraction and removal}: We extract and remove the text in the memes using open-source Python packages EasyOCR\footnote{https://github.com/JaidedAI/EasyOCR} and MMEditing\footnote{https://github.com/open-mmlab/mmediting}. The texts are removed from the memes to facilitate better entity and demographic detection.
    \item \textbf{Entity detection}: To augment the memes with relevant external information, we leverage Google Vision Web Entity Detection API\footnote{https://cloud.google.com/vision/docs/detecting-web} to detect and caption the entities in the cleaned image. The detected entities provide contextual information on the memes. 
    \item \textbf{Demographic detection}: Often, hate speeches are targeted at groups based on demographic information such as race and gender, and such information servers as important contextual information in hateful meme classification. To augment the memes with demographic information, we utilized the FairFace classifier~\cite{karkkainen2019fairface} to detect and classify the faces in the images, then mapping the label back to the person's bounding box with the largest overlapped area with the face. Noted that the demographic information is only extracted when the meme contains human entities.
\end{itemize}

The pre-processed datasets serve as input for the training of our proposed model discussed in the next section.


%Similar to Ron Zhu’s\cite{zhu2020enhance} point of view, though the analysis of the Hateful Memes\cite{kiela2020hateful} and MultiOFF\cite{suryawanshi2020multimodal} datasets, hateful elements often comes from gender, race ,religion,celebrities and historical events. It’s hard to rely on the model trained on the two datasets to identify and distinguish these information. At the beginning, we tried to collect 490 external images and texts to complement information referring to race, gender, religion, special events and things like gun, cigarette, and bomb. There is some but little improvement in performance because the supplementary data is not comprehensive enough and is relatively small in scale. Besides, the picture size of MultiOFF is unreasonable and both two datasets exist the problems that the pixel information is covered by text and part of the images are made up of several patches, which has influence on the image feature extraction. 

%We first resize the images proportionally to a minimum of 140 pixels and a maximum of 850 pixels. Then recognize, locate and remove texts on the images by using MMEDIT[?] and EasyOCR[?]. At last, we divided images into patches though MMEDIT and match the patches and texts in the same images according to the position information. Finally, the data is processed into clean images, clean patches and clean-patch text pairs and we apply FairFace\cite{} and Google Vision Web Entity Detection[?] on these processed data to provide external information for our model.

%\noindent \textbf{Image Cleaning}

%Using EasyOCR to detect position and contend of texts in the images. Then mask the pixels belonging to the 
%text areas and predict new pixels to obtain clean images. All subsequent operations like image feature extraction, entity detection and patch detection on the image are based on clean images. The improvement of performance by cleaning images is detailed in ?..

%\noindent \textbf{Patch Detection}

%Many images from both Hateful Memes and MultiOFF are stitched together by several patches, which influences the process of entity detection. And for some images, especially in Hateful Memes, each patch is given a sentence. So it’s unreasonable to deal with patch and sentences belonging to other patches in the same image equally. We utilize MMEDIT to divide images into patches and match the texts according to the positions.

%\noindent \textbf{Entity Detection}

%It is unrealistic to expect model trained on Hateful Memes or MultiOFF to recognize religion, changeable celebrities and historical events like Muslim, Trump, Mr. Bean and 911. Google Vision Web Entity Detection can match image with online images to acquire relative entities, which provides plenty of external information.

%\noindent \textbf{Face Detection}

%Similarly, race and gender information is hard to be learned by model trained on limited dataset. So we use FairFace to extract these kinds of information.

%\noindent \textbf{Feature Extraction}

%We use Faster R-CNN[??] to extract regions from original images and cleaned images.


==> MM21 - Disentangling Hate in Online Memes (Cam-Ready)/Related.tex <==
%Our proposed \textbf{the name of the model}. In this section, we give a retrospective 
%{\color{red} point out the challenge in hate speech detection and multimodal hate speech detection and how the disentanlged representation helps}
%\subsection{Hate Speech Detection}
%{\color{red} point out the importance of thet disentangled representations: understanding the target of the memes}

%We summarize and present the three groups of related works that informed our study. 

\subsection{Hate Speech Detection}
With the proliferation of social media and social platforms, automatic detection of hate speech has received considerable attention from the data mining, information retrieval, and natural language processing (NLP) research communities. Several text-based hate speech detection datasets~\cite{waseem2016hateful,ParkF17,DavidsonWMW17} have been released. Previous works exploit both machine learning based methods~\cite{xiang2012detecting,chen2012detecting,waseem2016you,nobata2016abusive,chatzakou2017mean} and deep learning based techniques to tackle the problem~\cite{cao2020deephate,djuric2015hate,mehdad2016characters,gamback2017using,badjatiya2017deep,grondahl2018all,zhang2018detecting}. The existing automated hate speech detection method has yielded good performance. However, most of the existing studies have focused on text-based hateful content, neglecting the rich multimedia user-generated content.

%The task of hate speech detection is even more challenge than toxic or abusive comment detection as hate speech not only involves abusive words but the abusive content should be targeting at an individual or a group of individuals~\cite{DavidsonWMW17,cambridge}. 
%However, most of existing works merely represent the text with a compact vector and feed it to the classifier for prediction without understanding what the piece of text is targeting at or whether there is a target.
%To the best of our knowledge, there has been no work implicitly or explicitly modeling the target of the hate speech, whereas having target groups or individuals is the most significant difference between hate speech and abusive or toxic language. In this work, we propose to model targets of hateful contents in the disentangled latent space.

%both hateful mems and multioff dataset paper write smt about this research field
\subsection{Multimodal Hate Speech}
%{\color{red} requires 1) target identifying: multimodal meme, what is targeting 2) external knowledge}
To address the gap in hate speech detection research, recent works have attempted to  explore multimodal hateful content classification tasks such as detecting online hateful memes~\cite{kiela2020hateful,lippe2020multimodal,velioglu2020detecting,muennighoff2020vilio,zhang2020hateful,das2020detecting,zhou2020multimodal}. The flourish of multimodal hateful meme detection studies could be attributed to the availability of several hateful memes datasets published in recent year~\cite{kiela2020hateful,suryawanshi2020multimodal,gomez2020exploring}. For instance, Facebook had proposed the \textit{Hateful Memes Challenge}\footnote{https://ai.facebook.com/blog/hateful-memes-challenge-and-data-set/}, which encouraged researchers to submit solutions to perform hateful memes classification~\cite{kiela2020hateful}. A dataset consists of 10K memes were published as part of the challenge, and the memes are specially constructed such that unimodal methods cannot yield good performance in this classification task. Therefore, existing studies have motivated to adopted a multimodal approach to perform hateful memes classification.

The existing multimodal hateful memes classification approaches can be broadly categorized into two groups: (a) models that adopt early fusion techniques to concatenate text and visual features for classification~\cite{suryawanshi2020multimodal,kiela2020hateful}, and (b) models that directly fine-tune large scale pre-trained multimodal models~\cite{kiela2020hateful,lippe2020multimodal,velioglu2020detecting,muennighoff2020vilio,zhang2020hateful,das2020detecting}. Recent studies have also attempted to use data augmentation~\cite{zhou2020multimodal,zhu2020enhance} and ensemble methods~\cite{sandulescu2020detecting,velioglu2020detecting} to enhance the hateful memes classification performance. Nevertheless, these existing methods have limited explainability and cannot reason the context embedded in the hateful memes. For example, hate speech should involve abusive content targeted at an individual or a group~\cite{awal2021angrybert,DavidsonWMW17,cambridge}. However, most hateful memes classification methods cannot identify the hate targets and unable to provide the context for the hateful content. %The closest work to identifying target entities in the hateful meme was proposed by \citet{zhu2020enhance}, where the researchers augment the memes with external general entity labels linked to general regions within the meme image. %However, the proposed method had augmented mostly general entities such as a `hat' or `shirt' that are less informative for hateful meme classification. %Furthermore, the augmented data are simply concatenated with the original hateful meme as input into the multimodal classification modal. 

This paper aims to address the research gaps by proposing a novel framework, \textsf{DisMultiHate}, which learns and disentangles the representations of hate speech-related target entities, such as race and gender, in memes to improve the hateful content classification. Unlike \cite{zhu2020enhance}, which augment general entities information as input, we extract the target entities using disentangled latent representations learned using self-supervised training. The disentangled representations serve as contextual information to provide some form of explanation to the hateful meme classification.  



%Previously, besides text-based classification, several datasets have been proposed focusing on classification tasks like multimodal sentiment analysis~\cite{hu2018multimodal,hu2018multimodal,zadeh2015micro,morency2011towards} and multimodal sarcasm detection~\cite{schifanella2016detecting,cai2019multi}. With the recent published datasets in multimodal hateful memes detection~\cite{kiela2020hateful,suryawanshi2020multimodal,gomez2020exploring}, hate speech detection in a multimodal setting becomes a focus of attention. Based on the text and the corresponding image, models are expected to make predictions whether the combination of them is hateful or not. Detecting hateful memes is challenging because it requires reasoning about subtle cues as well as understanding of background knowledge of the memes. On the other hand, models are easily confused by ``benign counfounders'' that flip the label of a multimodal hateful meme. Therefore, the capability of multimodal reasoning and comprehension is required. 

%Despite the difficulty of multimodal hateful memes detection, current models rely on early fusion techniques~\cite{suryawanshi2020multimodal,kiela2020hateful} or directly finetune large scale multimodal models~\cite{kiela2020hateful,lippe2020multimodal,velioglu2020detecting,muennighoff2020vilio,zhang2020hateful,das2020detecting,zhou2020multimodal}. 
%zhou2020multimodal: image captioning: multi task learning
%To enhance the performance of models, recent works utilize tricks such as ensemble~\cite{sandulescu2020detecting,velioglu2020detecting}, which is costly. Nonetheless, the potential of models themselves has not been explored well.

%{\color{red} should we emphasis this point here?}
%In this paper, we put forward a task specific solution for hateful memes detection in two aspects. Firstly, detecting hateful memes sometimes calls for the background knowledge. As a consequence, following~\cite{zhu2020enhance}, we extract entities, race and gender labels from the image and further extend the strategy to other datasets. Rather than blindly feeding all information into a multimodal pretrained model in ~\cite{zhu2020enhance}, we propose to extract the target of the multimodal meme using disentangled representations in the latent space with self-supervised training, which is crucial for hate speech detection as targeting at individuals is an unique characteristic of hateful content. Without relying on large scale any multimodal pretrained models, our proposed model surpasses all the other models on the hateful memes detection.
%{\color{red}will reviewers argue that why we haven't applied the disentangled part to multimodal pretrained models?}

\subsection{Disentangling Representation Learning}
\citet{bengio2013representation} defined a disentangled representation as one where single latent units are sensitive to changes in a single generative factor while being relatively invariant to changes in other factors. Hence, \cite{bengio2013representation} proposed to factorize and learn disentangled representations by training independent units to encode different aspects of input data. Various methods have also been proposed to perform representation disentanglement. For instance, existing studies have attempted to learn disentangled representations using supervised signals~\cite{hinton2011transforming,karaletsos2015bayesian,goroshin2015learning}. Other works have explored purely unsupervised approaches to disentangled factor learning by exploiting the information-theoretic aspect of the variational auto-encoders and adding a regularization term that minimizes the mutual information between different units of the representations~\cite{burgess2018understanding,chen2018isolating,HigginsMPBGBML17}.

Latent representation disentanglement has been applied in various tasks. For example, representation disentanglement had been applied to learn and disentangle users' preferences for different categories of items to improve recommendation~\cite{ma2020disentangled,ma2019learning}. \citet{bouchacourt2018multi} had exploited the disentangled representation learning to group data based on disentangled visual semantics. \citet{dupont2018learning} had disentangled representations to learn factors that correspond to handwriting numbers' various characteristics. This paper contributes the state-of-the-art in disentangled representation learning by disentangling the representation of target entities in online hateful memes. To the best of our knowledge, this is the first work that applies representation disentanglement on the hateful memes classification task.


%According to the definition in~\cite{bengio2013representation}, a disentangled representation is the one where single latent units are sensitive to changes in single generative factors, while being relatively invariant to changes in other factors. As a consequence, a disentangled representation is factorised and independent units learn to encode different independent aspect of input data. Various methods have been proposed to force the disentanglement of representations. Some works to learn disentangled representations requires supervised signals~\cite{hinton2011transforming,karaletsos2015bayesian,goroshin2015learning}. There are also purely unsupervised approaches to disentangled factor learning, for instance those exploiting the information-theoretic aspect of the variational auto-encoders and adding a regularization term which minimizes the mutual information between different units of the representation~\cite{burgess2018understanding,chen2018isolating,HigginsMPBGBML17}. The idea of disentangled representation learning has also been applied to various tasks where each unit in the disentangled representation has task-specific meaning. For example, for the task of recommendation, each unit in the disentangled latent space represents users' preference under different categories of items~\cite{ma2020disentangled,ma2019learning}; in~\cite{bouchacourt2018multi}, the author exploited the disentangled representation learning which groups data based on visual semantics and in~\cite{dupont2018learning}, each element in the disentangled representation corresponds to some characteristics of the handwriting numbers.

%To our knowledge, we are the first proposing to use disentangled representations in hate speech detection and use the representation figure out targets of hateful contents which aids the task .

